Constructing Light Spanners Deterministically in Near-Linear Time

Graph spanners are well-studied and widely used both in theory and practice. In a recent breakthrough, Chechik and Wulff-Nilsen [CW18] improved the state-of-the-art for light spanners by constructing a $(2k-1)(1+\epsilon)$-spanner with $O(n^{1+1/k})$ edges and $O_\epsilon(n^{1/k})$ lightness. Soon after, Filtser and Solomon [FS19] showed that the classic greedy spanner construction achieves the same bounds The major drawback of the greedy spanner is its running time of $O(mn^{1+1/k})$ (which is faster than [CW16]). This makes the construction impractical even for graphs of moderate size. Much faster spanner constructions do exist but they only achieve lightness $\Omega_\epsilon(kn^{1/k})$, even when randomization is used. The contribution of this paper is deterministic spanner constructions that are fast, and achieve similar bounds as the state-of-the-art slower constructions. Our first result is an $O_\epsilon(n^{2+1/k+\epsilon'})$ time spanner construction which achieves the state-of-the-art bounds. Our second result is an $O_\epsilon(m + n\log n)$ time construction of a spanner with $(2k-1)(1+\epsilon)$ stretch, $O(\log k\cdot n^{1+1/k})$ edges and $O_\epsilon(\log k\cdot n^{1/k})$ lightness. This is an exponential improvement in the dependence on $k$ compared to the previous result with such running time. Finally, for the important special case where $k=\log n$, for every constant $\epsilon>0$, we provide an $O(m+n^{1+\epsilon})$ time construction that produces an $O(\log n)$-spanner with $O(n)$ edges and $O(1)$ lightness which is asymptotically optimal. This is the first known sub-quadratic construction of such a spanner for any $k = \omega(1)$. To achieve our constructions, we show a novel deterministic incremental approximate distance oracle, which may be of independent interest.

==> ado.tex <==

\section{Improving the preprocessing time of approximate distance
oracles}\label{sec:ado}
%\todo{Referer til dette appendix i afsnit~\ref{sec:sort}; brug Baswana-Sen i stedet for vores Greedy; fjern tabel; $O(\log k)$ query-tid kan opnås; citer Shiris to seneste do-artikler.}

In~\cite{CWN12,DBLP:conf/soda/Wulff-Nilsen13}, it was shown how to compute a distance oracle with stretch $2k-1$, space $O(kn^{1+1/k})$, and query time $O(\log k)$ in time $O(\sqrt{k}m + kn^{1 + c'/\sqrt{k}})$ for a constant $c'$. While constructions exist with better space and query time~\cite{Chechik14,Chechik15} when $k = \omega(1)$, these constructions have worse preprocessing time. We show how to use the trick from Section~\ref{sec:sort} in the framework of~\cite{CWN12,DBLP:conf/soda/Wulff-Nilsen13} to remove the factor $O(\sqrt{k})$ from the first term in the preprocessing time while only increasing the preprocessing time by a term of order $\sqrt kn^{1+\eps}$ and by a constant factor increase in $c'$, where $\eps > 0$ is a constant that can be chosen arbitrarily small. This gives linear preprocessing time for all but the sparsest graphs.

The observation behind the result is that the original invocation of the algorithm of Baswana and Sen from the construction of~\cite{CWN12,DBLP:conf/soda/Wulff-Nilsen13} can be replaced by \emph{two} invocations of this algorithm. The first invocation is with $2/\eps - 1 = O(1)$ stretch. The second is invoked upon the first spanner with $O(\sqrt{k})$ stretch. The result is a spanner whose stretch is the product of the two, i.e., it has stretch $O(\sqrt k)$ as needed in~\cite{CWN12,DBLP:conf/soda/Wulff-Nilsen13}. A single invocation of Baswana and Sen providing $O(\sqrt{k})$ stretch takes time $O(\sqrt{k}m)$, giving the first term in the preprocessing of~\cite{CWN12,DBLP:conf/soda/Wulff-Nilsen13}, whereas the double-invocation takes time \[ O\left( \frac{1}{\eps} m + \frac{\sqrt{k}}{\eps}n^{1+\eps} \right) = O \left(m + \sqrt k n^{1+\eps}\right) \text{.}\]  
%We note that our new spanner from \Cref{thm:fast_greedy} can be used in the same manner, which would save the factor of $O(\sqrt{k})$ from the second term in the above, however due to $k \leq \log n$ this has no impact asymptotically.

\begin{theorem}\label{thm:fastoracle}
    Let $G$ be an undirected edge-weighted graph with $m$ edges and $n$ vertices and let $k$ be
    a positive integer. Then for any fixed constant $\eps > 0$ there exists a constant
    $c = \frac{4\sqrt{6}}{\eps} - 2 \sqrt{6}$, such that one can construct a $(2k-1)$-ADO for $G$ of size
    $O(kn^{1+1/k})$ with query time $O(\log k)$ in time
    \[
        O\!\left(
        m + \sqrt k n^{1+\eps} + kn^{1+c/\sqrt{k}} 
        \right)\ .
    \]
%    be an integer, and fix $0 < \eps \leq 1$ such that $1/\eps$ is integer.
%    There exists a constant $c' > 0$ such that an $2k-1$-approximate distance
%    oracle for $G$ of size $O \left(kn^{1+1/k}\right)$ can be constructed in
%    time $O\left(m + \sqrt{k}n^{1+ \eps + c'/\sqrt{k}} + kn^{1 + c/\sqrt{k}}
%    \right)$, and the oracle has query time $O(k)$.
\end{theorem}

%and insert it directly into the approximate distance oracle construction of
%Wulff-Nilsen~\cite[Theorem 3]{CWN12}. Our spanner replaces Baswana and
%Sen~\cite{BaswanaS07}, and a consequence of the optimal size of our spanner
%along with its fast construction time is that the approximate distance oracle
%preprocessing takes a factor of $O(\sqrt{k})$ less. See \Cref{tab:oracles} for
%related distance oracle constructions. We get the following theorem.


%    In particular, if $k = \omega(1)$ we obtain a running time of $O(m +
%    n^{1+\eps})$, which is linear for all but very sparse graphs.

% \begin{table*}[h]
%     \small
%     \centering
%     \makebox[0pt][c]{
%         \begin{tabular}{c|c|c|c|c}
%             \toprule

%             \bf Stretch & \bf Space & \bf Query & \bf Preprocessing & \bf Ref\\
%             \midrule
%             $2k-1$&   $O \left(kn^{1+1/k} \right)$ & $O(k)$ &$O \left(kmn^{1+1/k} \right)$ & \cite{ThorupZ05} \\
%             $2k-1$&   $O \left(kn^{1+1/k} \right)$ & $O(k)$ &$O \left( \min \{n^2, kmn^{1+1/k}\} \right)$ & \cite{BaswanaKMP05} \\
%             $2k-1$&   $O \left(kn^{1+1/k} \right)$ & $O(k)$ &$O \left(\sqrt{k}m + kn^{1+\frac{c'}{\sqrt{k}}} \right)$ & \cite{CWN12} \\
%             $O(k)$&   $O \left(n^{1+1/k} \right)$ & $O(1)$ &$O \left( n^{2+1/k}
%             \log n\right)$ & \cite{MendelN06} \\
%             $O(k)$&   $O \left(kn^{1+1/k} \right)$ & $O(k)$ & $O\left(m + kn^{1+1/k+\eps} \right)$ & \cite{CWN12}\\
%             \midrule
%             $2k-1$&   $O \left(kn^{1+1/k} \right)$ & $O(k)$ &$O \left(m + \sqrt{k}n^{1+\eps+\frac{c}{\sqrt{k}}} \right)$ & \Cref{thm:fastoracle} \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{Table of related stretch $2k-1$ and $O(k)$ distance oracle constructions.}
%     \label[table]{tab:oracles}
% \end{table*}

\begin{proof}
We note that the construction and thus proof is the same as \cite[Theorem
3]{CWN12} (the improvement in query time to $O(\log k)$ in~\cite{DBLP:conf/soda/Wulff-Nilsen13} does not increase the asymptotic preprocessing time) so we only highlight the differences in the
preprocessing time analysis. We assume, as in~\cite{CWN12}, that $k$ is bounded from below by a sufficiently large constant. This can be done without loss of generality since if for constant $c''$ it holds that if $k \leq c''$ then the construction of \cite{CWN12} already gives the desired preprocessing time bound.

Let $c'$ be the constant used to bound the running time in \cite[Theorem 3]{CWN12} and $k' = 2 \sqrt{k}/c$. We will argue that picking $c = c'(2\eps-1)$ and using the double-invocation of Baswana and Sen's construction gives~\Cref{thm:fastoracle}. The preprocessing in~\cite{CWN12} consists of the following three components:
\begin{enumerate}
\item Constructing a Thorup-Zwick oracle on a graph $G_S = (V,E_S)$ defined by a subset $S$ of randomly sampled vertices.
\item Constructing a $(2k'-1)$-spanner $H$ of $G$ where $k' = \Theta(\sqrt k)$.
\item Constructing a restricted Thorup-Zwick oracle on $H$ with stretch $2\kappa - 1 = \Theta(\sqrt k)$.
\end{enumerate}

Only the two latter components give rise to the $\sqrt k m$-term so we only focus on these in the following.

We modify the second step so that it constructs a $(2\eps -1)(2k'-1)$-spanner $H$ using the double-invocation of Baswana and Sen. As shown above, this can be done in time $O\left(m + \sqrt k n^{1 + \eps}\right)$. The size of $H$
is $h = O \left(k'n^{1 + 1/k'}\right)$. It follows from the
proof of \cite[Theorem 3]{CWN12}, that the constant $c'$ can be picked
to be a factor $2\eps -1$ larger than the $c$ in the original analysis, i.e., we pick $c = c'(2\eps -1)  = 4\sqrt{6} / \eps - 2 \sqrt{6}$.

In the third step, we construct a $(2\kappa-1)$-approximate Thorup-Zwick oracle on $H$ restricted to $S$, meaning we only store bunches for vertices $v \in S$. The preprocessing time of Thorup-Zwick is then $O \left(\kappa k' n^{1 + 1/k' + 1/\kappa} \right)$.

Total preprocessing for the two steps is thus
\[
  O \left(m +  \sqrt k n^{1 + \eps} + \kappa k' n^{1 + 1/k' + 1/\kappa} \right),
\]
and by the choices of $k'$ and $\kappa$ the theorem follows.
\end{proof}

